Some Languages are More Equal than Others: Probing Deeper into the Linguistic Disparity in the NLP World

Linguistic disparity in the NLP world is a problem that has been widely acknowledged recently. However, different facets of this problem, or the reasons behind this disparity are seldom discussed within the NLP community. This paper provides a comprehensive analysis of the disparity that exists within the languages of the world. We show that simply categorising languages considering data availability may not be always correct. Using an existing language categorisation based on speaker population and vitality, we analyse the distribution of language data resources, amount of NLP/CL research, inclusion in multilingual web-based platforms and the inclusion in pre-trained multilingual models. We show that many languages do not get covered in these resources or platforms, and even within the languages belonging to the same language group, there is wide disparity. We analyse the impact of family, geographical location, GDP and the speaker population of languages and provide possible reasons for this disparity, along with some suggestions to overcome the same.

==> Instructions.tex <==
\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}


\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> Removed.tex <==
%https://arxiv.org/pdf/2012.15613.pdf

%https://arxiv.org/pdf/2104.08726.pdf  - small dataset for truly LR languages

%https://arxiv.org/pdf/2005.09093.pdf - include your language data in UD, etc, and models will be tested by others for your languages

%NAACL Emerging Regions Fund

%https://arxiv.org/pdf/2005.09093.pdf show low-resource languages benefit from multilingual joint training, as bilingual BERT outperforms monoling

%http://proceedings.mlr.press/v119/hu20b/hu20b.pdf   - assumes monolingual data is available. Use amount of wiki data as a measurement of unannotatead data

%https://arxiv.org/pdf/2005.00633.pdf - even little bit of annotatead data helps

%https://arxiv.org/pdf/2010.14571.pdf - data for thousands of languages


%https://aclanthology.org/2020.repl4nlp-1.16.pdf - Our findings suggest, with small monolingual corpus, BERT does not learn high-quality representation for low resource languages. To learn better representation for low resource languages, we suggest either collect more data to make low resource language high resource (Conneau et al., 2019), or consider more data-efficient pretraining techniques like Clark et al. (2020). Also say bilingual training helps, when there is not enough data to train monolingual model.


%https://arxiv.org/pdf/2012.15613.pdf - monolingual tokenizers are typically trained by native-speaking experts who are aware of relevant linguistic phenomena exhibited by their target language.

%more D\&I efforts.\\

%https://aclanthology.org/2021.sigtyp-1.7.pdf - inportance of quic translation
%\end{itemize}







%As far as we are aware, this is the most recent language categorisation. Since the basis is the amount of language resource available for a language, it is a more meaningful metric to evaluate the status of languages with respect to NLP techniques that rely on data.

%However, we note multiple issues with this categorisation. First and foremost, we note that considering only LDC and LREC effectively omits a vast pool of resources that are available in shared tasks as well as in public github repositories. In particular, researchers working with low-resource languages may not have submitted their datasets to LDC and LREC venues simply because of lack of awareness or due to the proprietary nature of data. We also note that progress of NLP with respect to a language should not be quantified only with respect to the language resources, but also with respect to the number of researchers actively working on a given language and the amount of publications coming out for that language. 

%We also note that considering these criteria in a language categorisation across thousands of languages is not feasible, which leads us to our initial argument - in documenting the language resources and amount of research conduced per language, a major role should be played by the researchers who use, or are familiar with that language. Having said that, we are not aware of any systematic studies that carried out to identify the status of a language with respect to these factors.

%In this research, we use Sinhala as a usecase and empirically show the importance of per-language efforts to document the status of a language. In fact, the category assigned to Sinhala in \citet{joshi-etal-2020-state}'s categorisation is ambiguous. While Sinhala is placed in category 0, its synonymous term Sinhalese is placed in category 1. Specifically, we show that Sinhala does contain a vast number of language resources scattered around, although none was included in  LDC and LREC. We also point to multiple multilingual corpora where Sinhala is included, something that has been overlooked by \citet{joshi-etal-2020-state}. Thus, we note that categorising languages with respect to the available data sources can be highly misleading as a common scale cannot be identified across all the languages.  Further we note that considering the data in wikipedia only is not adequate, since most of the language data is now generated within news sites and social media sites. We show that considering CC statistics would be a better indicator.

%We carry out a comparative analysis wrt to the amount of publications per language, and show that Sinhala indeed has a considerable amount of publications and is an outlier for class 0 and 1.


%We also have a close look at the research conducted for Sinhala so far, and derive multiple observations that explain why Sinhala is considered as a low-resource language while it has been categorised as an institutional language in the ethnology []. Based on these observations, we bring out multiple recommendations that might help to more the current low-resource languages out of their low-resource status.

%As mentioned above, we note that the status of a particular language can be better documented by researchers working on that language. As an attempt to help them in this, we publicly release the code and scripts we used for the analysis of Sinhala. If the same analysis can be conducted by individual researchers on their languages, hopefully, in the future, we would have a better picture of the true status of the languages with respect to the language resources and amount of research. 

%\section{Research Questions}
%\begin{enumerate}
%\item Is it possible to categorise languages wrt the amount of language resources available?
%Our argument and experiments: Derive the relationship between population of speakers and the amount of unannoated data. Show how much language resources that Sinhala has. and present it as a counter example to show that considering LRE and LDC is not accurate. Also can try to find out why people are not submitting to LDC and LRE. Then compare CC and wikipedia stats to see which is better. should parallel data stats be considered? Also bring out the argument that individual researchers should start documenting the resources for their languages.

%\item What other factors should be considered to categorise languages?
%Our argument and experiments - get stats from google scholar on the number of research papers and check if the findings correlate with Joshi's categorisation

%inclusion in google translate, FB translate, google input tools etc?

%Inclusion in pre-trained language models? Availability of pre-trained models in hugginface, etc?

%\item Where do low-resource language researchers publish?
%Can analyse wrt Sinhala survey paper. And can see if any other survey paper can be found for other languages (Hindi one is already there, but would be too daunting)

%\item Why low-resource languages continue to be low resource? Can derive insights from our survey paper and show e.g. no collaboration, less sharing of data and code, not maintaining websites, etc. Can show the Mazakane project as a positive development for African languages.

%\item whta techniques specific for LR languages have been applied on LR languages?

%\end{enumerate}

%\section{Introduction}

%\textbf{options for Google search}:
%\begin{enumerate}
%    \item as done in https://arxiv.org/pdf/2005.00633.pdf, some lower-level structured prediction tasks: POStagging, dependency parsing, and NER, and some higher-level language understanding tasks: NLI, and QA, classification, translation.
%\item http://proceedings.mlr.press/v119/hu20b/hu20b.pdf has a classification of four tasks:

%classification - natural language inference, paraphrase identification

%structured predication - POS, NER

%question answering

%Retrieval - parallel sentence extraction 

%A good categoration in https://arxiv.org/pdf/2010.12309.pdf they refered to the wikipedia page on NLP


%interesting fact - \cite{cieri2016selection} claims that Arabic and Chinese were severly under-resourced at the begining of the millennium. 

%http://ciir.cs.umass.edu/pubfiles/ir-312.pdf



%categorisation in papers with code: %https://paperswithcode.com/area/natural-language-processing




%Over the years, there have been many initiatives to categorise languages according to the aforementioned different criteria~\cite{harmon1995status,joshi-etal-2020-state}. Given that the category of a language may change with time, we rely on the language categorization  recently proposed by \citet{joshi-etal-2020-state} to identify LRLs. As shown in Table~\ref{tab:language_categories},~\citet{joshi-etal-2020-state} categorised 2485 languages into six groups based on the amount of publicly available data.

%===========================================
%Sinhala is an Indo-Aryan language primarily used by a population of about 16M in the island nation of Sri Lanka. Despite being an Indic language, which has close ties to major Indian languages such as Hindi, Sinhala was not included in any of the language computing initiatives in India. This, and many other factors such as the economic setbacks in the country slowed down the development of Sinhala language computing tools. Consequently, Sinhala is labelled as a low-resource language. In fact, it has been considered as a use-case for low-resource languages in multiple research [Guzman's paper, and some other NMT papers]. In the recent language categorization of \citet{joshi-etal-2020-state}, which groups language into 6 categories (0- extremely low-resource, 5- high-resource), the exact position of Sinhala is not clear - Sinhala is put into category 0, while its synonymous term Sinhalese is put into category 1. Despite this ambiguity, this categorisation clearly indicates that Sinhala is a low-resource language.

%However, \citet{joshi-etal-2020-state} consider only two factors in determining the language category - the availability of annotated data for a language in LDC and ELRA, and the amount of wikipedia data as un-annotated data. However, the resourcefulness of a language can be analysed with respect to multiple other factors such as the number of people speaking that language, amount of research conducted....... [cite]. On top of that, the future state of language research depends on the number of researchers actively working on the said language. 

%In this paper, we use Sinhala as a usecase and show that the category of a language actually changes with respect to these different factors. In fact, other than few research [cite]  that analised the plight of languages in a holistic manner, we are not aware of any research that deeply analysed a selected language wrt these multiple factors. For many low-resource languages, such an analysis will provide very valuable insights into the current status of the language. The code and scripts we developed during this analysis is publicly released to be used for any other language with minimal editing.

%Other than this quantitative analysis, we conducted a qualitative analysis of Sinhala language computing. While briefly summarising the Sinhala language computing research conducted so far, we make very valuable observations, which we believe would be common for many other low-resource languages. Based on these observations, we make some general recommendations to push low-resource languages out of their low-resource status.


%https://www.ethnologue.com/size-and-vitality/sin

%https://glottolog.org/glottolog/language

%can compare the status of Sinhala related NLP techniques against this - https://arxiv.org/pdf/2010.12309.pdf

%http://proceedings.mlr.press/v119/hu20b/hu20b.pdf

%https://arxiv.org/pdf/2006.07264.pdf

%https://thegradient.pub/the-benderrule-on-naming-the-languages-we-study-and-why-it-matters/
%================================

%Need to identify the usecase that Sinhala represents - an insular language, which never got included in language group-wise research (e.g. Masakhane project in Africa, or Europarl project in Europe, or the projects sponsored by the Indian government). Sinhala is a well-developed language, active user community. Literacy rate among the Sinhala speaking people is very high (at 96.4 against a national average of 79.7~\cite{department2012Census}). Computer literacy is also high (See Table~\ref{tab:itLit}). During the early times of the Unicode project, Sinhala managed to get its Unicode system. So digital content is widely available, although not as much as for English (can refer to CC stats). But the problem is annotated/parallel data.

%According to \citet{joshi-etal-2020-state}'s categorization, Sinhala belongs to class 0, meaning that it has exceptionally limited resources. They looked at resources in places s.a. LDC, and no Sinhala data are there.

%However, according to \citet{ranathunga2021neural} wrt NMT research, Sinhala is an outlier in this class 0. Reason is the FLORES and OPUS datasets that include Sinhala. Many NMT research has used  these datasets for NMT research, and there have been WMT shared tasks on these datasets. This shows the importance of sharing resources for a development of NLP research on a language. Can add corpora list from the survey

%\citet{bhattacharyya2019indic} discussed common problems in Indic Language computing. Can expand on this and highlight Sinhala-specific challenges.

\iffalse
Problems identified by \citet{de2021survey}:
\begin{enumerate}
    \item Duplicate research efforts: e.g. During the same time, two Sinhala WordNet projects. Even after some time because it seems people are either not reading other groups' papers or reluctant to build on them
    \item Created data not being released
    \item implemented systems abandoned after some time
    \item Sinhala language knowledge is still in books, guarded by copyright laws
\end{enumerate}

other points:
Sinhala data not being contributed to shared repositories. e.g. no sinhala data in the Universal Dependency project.~\citet{caswell2021quality} notes how weak the parallel corpora are (including Sinhala).


Positive points:
\begin{enumerate}
    \item Sinhala is included in XLM-R, LABSE, mBART, LASER and mT5. This is a very useful thing. Facebook has Sinhala fastText embeddings.  Already local researchers have reaped the benefits of this (MERCon paper on mBART to appear). What is your FastText paper? (I have a comment on my survery "cite FastText paper")
    \item Sinhala datasets created by international research projects
\end{enumerate}

Insights we can derive from \cite{de2021survey}:
1. Time taken to apply new techniques on Sinhala. e.g. Word2Vec was introduced in 2013, but first research on Sinhala Word2Vec came in 2020.
In contrast mBART was introduced in 2019, and first mBART related Sinhala paper came in 2021.

Amount of papers per NLP task, and how this number varies with year.

Identify a commonly accepted NLP task list and show for which tasks no Sinhala research is available. We do have the subsections of the survey. 

Identify some other languages in the class 0 category, and compare the amounts of research papers.


Sinhala text processing systems available:
Made by SL researchers: SiTa NMT system, Subasa, Helakuru

Included in other systems: Google translate, Google input tools, Facebook translate

Sinhala datasets available: By Sinhala NLP researchers, by others, what is publicly available?

There is a Hindi survey https://arxiv.org/ftp/arxiv/papers/2102/2102.00214.pdf
\fi
% Nisansa TODO
%(done)share paper folder
%(done)paper coount fre qncy graph
%(done) anthology -> Sinhala
%(done) If possible abstract
%(done) Get the josh list excel sheet
%(done) Run ACL count for All joshi langs 
% (done) Get the list with " | etc
% (done) Do the paper source trends graph using the excel sheet and years (See the one  in images)
% (done) https://commoncrawl.github.io/cc-crawl-statistics/plots/languages
% (done) https://meta.wikimedia.org/wiki/List_of_Wikipedias
% (done) parallel corpus (also total count)
% (done) Fix the "where_published" issue
% (done) read Joshi's ACL anthology section (Embedding on anthology)
% (done)  get OPUS list
%  (done) Get OPUS sentence number
% draw graphs for https://docs.google.com/spreadsheets/d/1w3rLszUF8JGYt3mh9qQmsvbdpOtkcgQoMLq_StaZruM/edit#gid=00
%  (done)  Run ACL code for new lang list
%  (done)  Get some dummy data set and do the bubble graph
%  (done)  Get full data set and do the bubble graph
% (done) howw many ethnalog classes in every class
% (Done) Normalize aove with pop size add column
% (Done) Fb to lang % : Contri  {tab:ConAndCov}
% (Done) Lang to FB %: Covera {tab:ConAndCov}
% (done) year wise ACL graph for 12 categories  {fig:ACLall}


%\SurveyGraph{code_available}{Code Availability}
%\SurveyGraph{data_available}{Data Availability}
%\SurveyGraph{tool_publicly_available}{Tool Availability}
%\SurveyGraph{language}{Used Language}
%\SurveyGraph{where_published}{Where the papers were published}


























%\section{Corpora}

%For NLP research in any language the availability of corpora plays large part. The general, corpora can either be \textit{monolingual} or \textit{multilingual}. In that latter case, the corpus may also be called \textit{parallel} or \textit{aligned}. The Table~\ref{tab:corpora} provides a summery of the available Sinhala Corpora.

%The most common and largest type of language corpora are usually \textit{monolingual}. This is because collecting a monolingual corpus consists of the relatively easier task of crawling the web or OCR; both of which can be done by computer scientists without the help of a language specialist. However, we notice that in Sinhala, researchers opt to collect \textit{multilingual} corpora rather than monolingual ones. 

%\subsection{Sinhala Monolingual Corpora}
%The oldest reference to a Sinhala monolingual corpus we have found is the work by~\citet{weerasinghe-etal-2009-corpus} where they claim to have created a word corpus of approximately 35,000 entries. However, according to~\citet{de2019survey}, this corpus is no longer publicly available. The oldest publicly available\footURL{https://osf.io/a5quv/} large Sinhala monolingual corpus is the web crawled corpus created by~\citet{upeksha2015implementing,upeksha2015comparison}. 
%
%The very small web crawled Sinhala news corpus\footURL{https://osf.io/tdb84/} by~\citet{de2015Sinhala} has the data classified under the labels: \textit{business}, \textit{entertainment}, \textit{politics}, \textit{science and technology}, and \textit{sports}.
%
%Even though~\citet{wijeratne2020sinhala} initially released\footURL{https://bit.ly/2GEI4d6} a corpus compiled from a decade of Sinhala Facebook posts, they have now taken the corpus offline with only the stop words list that they generated from the corpus remaining available. 
%

%\subsection{Sinhala Multilingual Corpora}
%The open parallel corpus project\footURLcl{https://opus.nlpl.eu/}{opus} by~\citet{tiedemann2012parallel} hosts a number of Sinhala parallel corpora obtained from various open source localization data: \textit{Mozilla-I10n}, \textit{GNOME}, \textit{KDE}, and \textit{Ubuntu}. It also contains a \textit{wikimedia} data set published by the wikimedia foundation and their article translation system. The \textit{WikiMatrix}~\cite{schwenk2021wikimatrix} compiled by \textit{Facebook Research} is also based on wikimedia.

%A popular source for Sinhala parallel corpora are subtitle files. The open parallel corpus project\cref{opus} also hosts a number of such data sets. The \textit{QED}~\cite{abdelali2014amara} data set is based on the QCRI Educational Domain Corpus which is an open multilingual collection of subtitles for educational videos and lectures. The \textit{OpenSubtitles}~\cite{lison2018opensubtitles2018} data set, as the name suggests, was developed by automatically aligning the lines in files from the open subtitles website. The \textit{TED2020}~\cite{reimers-gurevych-2020-making} data set is a collection of TED and TED-X transcripts. 

%\cite{guzman2019flores} is unique among parallel corpora given that it contains 8569 professionally translated parallel sentences from wikipedia. Web crawling is another popular way used to generate Sinhala parallel corpora hosted at the open parallel corpus project\cref{opus}. \textit{ParaCrawl}~\cite{banon2020paracrawl} data set has been created by automatically aligning the results of a general web crawl. However, the later study by~\citet{caswell2021quality} claims that upon inspection, only 37.00\% of the data were correctly aligned and translated. \textit{CCAligned}~\cite{el-kishky-etal-2020-ccaligned} data set was created from \textit{Commoncrawl} Snapshots while margin-based bitext mining techniques were used to \textit{CCMatrix}~\cite{fan2021beyond} web crawl. The JW300~\cite{agic-vulic-2019-jw300} data set uses a limited web crawl restricted to the official \textit{Jehovah’s Witnesses (jw.org)} website. \textit{XLEnt}~\cite{el2021xlent} brings together \textit{WikiMatrix}, \textit{CCMatrix}, and \textit{CCAligned} to obtain entity pairs. This was obtained by performing named entity recognition and typing on English sentences, labels of which were then projected on-English aligned sentence pairs. 


% To Do (Copy-pasted from survey)
%%A parallel corpus\footURL{https://github.com/kdissa/comparable-corpus} of aligned Sinhala-English documents and sentences obtained from crawling the web was released by~\citet{sachintha2021exploiting}.


% Tamil and etc (Copy-pasted from survey)
%As for Sinhala-Tamil corpora,~\citet{hameed2016automatic} claim to have built a sentence aligned Sinhala-Tamil parallel corpus and~\citet{mohamed2017automatic} claim to have built a word aligned Sinhala-Tamil parallel corpus. However, at the time of writing this paper, neither of them was publicly available. A very small Sinhala-Tamil aligned parallel corpus created by~\citet{farhath2018improving} using order papers of government of Sri Lanka is available to download\footURL{http://bit.ly/2HTMEme}. A Sinhala and Tamil annotated corpus for emotion analysis was created by~\citet{jenarthanan2019actsea}. 
 
%Even after more than 60 years of existence, the fields of Computational Linguistics (CL) and Natural Language Processing (NLP) are still heavily biased towards a handful of so-called `high-recourse' languages.\blfootnote{\noindent The paper title is inspired by the quote ``\textit{All animals are equal, but some animals are more equal than others}'' by~\citet{orwell1945animal} which satirically alludes to disparities that exist in places which, ostensibly are supposed to be homogeneous. In this paper, we discuss how the same phenomenon is observed in the broadly used language categorisation systems.} This means that, most of the 6500+ languages in the world, which have been classified as `low-resource' have received limited to no attention from the CL and NLP community. This in turn, deprives billions of the world's population from reaping the benefits of the developments in the fields of CL and NLP.  
%For example, availability of certain language technologies would enable governments and other entities to provide better situation awareness at the time of a disaster, and help document the cultural and scientific information of the associated languages~\cite{cieri2016selection}.

%\section{NLP and CL Tasks}
%\subsection{Tools for Lower Levels of Language Analysis}
%By lower levels, we refer to tasks such as morphological analysis, parts of speech tagging and grammar parsing, which require language-specific knowledge. 

%According to Table xx, the amount of research conducted for these tasks is much lower compared to the end-user NLP applications. As This is partly due to the morphological complexity of the language, and lack of agreement on the corresponding language rules among the Sinhala scholars [need to find examples of disagreement is possible]. Most of the knowledge is locked down in old books. Some research has tried to document the morphological rules in a computer understandable manner, however these efforts are not comprehensive []. Consequently, the available morphological analysers do not cover all the possible rules of the language []. Out of these, only [x] has a working product.

%The same fate can be observed for POS tagging. Sinhala POS tags do have some overlap with the standard Indic POS tag set [], however, it has its unique POS rules. There have been two attempts to defined Sinhala POS tag sets, however both have their own limitations [xxx list limitations]. Some Machine Learning POS taggers are publicly available, however their accuracy is very much sub-optimal.

%The lack of grounded research for morphological analysis and POS seems to have had a cascading effect of grammar parsing. We are not aware of any working grammar parser for Sinhala. However some publications on developing CFG grammar [] as well as grammar parsing has been reported [].

%\subsection{Information Extraction}
%As for IE, we are aware of multiple research on Named Entity Recognition. However, except for the work of Azees [], others are based on a very small number of NE tags []. Out of these only Manaminee's data and code are available [].

%\subsection{Text Classification}
%Compared to other tasks, text classification has a noticeable amount of reported work []. Most notably, on top of the traditional classifiers such as Naive Bayes, SVM, much recent research has shown very impressive results with the use of neural word embeddings and recurrent NN models []. Out of the text classification tasks, sentiment analysis has been the most studied one. 

%\subsection{Semantic Tools}
%A handful of research is available for semantic similarity measurement [], text summarization [], word sense disambiguation []. However, none of this research has prolonged, nor tried out any recent Deep Learning based techniques. 

%\subsection{Machine Translation}
%Machine Translation is the NLP task that has been researched most wrt Sinhala. This is not surprising, because in Sri Lanka there are three official languages and it is required to translate all government documents into all the three languages. And MT seems to be the only NLP task that received the attention and funding from the government institutions.  MT research is mainly for Sinhala-English, and Sinhala-Tamil, with a very few for Japanese-Sinhala.\\
%Early research started with simple rule-based translation. Subsequent work reported the use of SMT. More recently, recurrent, as well as Transformer models have been used. The best result to date has been reported with the use of a pre-trained multilingual denoised sequence-to-sequence model (mBART).


%\subsection{Spell and Grammar Checkers}
%Early versions of grammar checkers were all based on rule-based and dictionary based techniques. Very recently, xx presented neural spell checkers for Sinhala, which outperformed these rule-based techniques by a large margin.xx's tool is available via a web interface, and yy's data and source code are publicly available.

%\subsection{OCR}

%\subsection{Miscellaneous Applications}
%There have been one or two research published for tasks such as text generation and chatbots. 

\iffalse
\subsection{Observations}
\begin{itemize}
    \item Only xx\% of the published work has code publicly available
    \item Only xx\% tasks have at least one publicly accessible working system
    \item Only xx\% of work related data/rule sets publicly available
    \item Except for text classification and MT, there seems to be no prolonged research efforts
    \item For many NLP tasks such as co-reference resolution, text simplification, x,y,z no research has been conducted.  
    \item Except for text classification, MT and xxx no deep learning based state-of-the art research has been carried out for Sinhala
\end{itemize}

\begin{table}
\centering
\begin{tabular}{lcc}
\hline
\multirow{2}{*}{\textbf{NLP Task}} & \multicolumn{2}{c}{\textbf{Research Count}}  \\
\hhline{~--}
& \textbf{Sinhala} & \textbf{Total}\\
\hline
POS Tagging & 1960 & 145k \\
Morphological Analysis & 3570 & 3930k\\
Text Classification & 3820 & 5160k \\
Machine Translation & 1980 & 3590k\\
\end{tabular}
\caption{Amount of research papers}
\label{tab:accents}
\end{table}


\begin{table}[!htb]
    \centering
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        First Language & 2017 & 2018 & 2019 & 2020 \\
        \hline
        Sinhala & 35.4 & 36.1 & 38.1 & 39.7 \\
        \hline
        Tamil & 27.7 & 29.8 & 30.8 & 33.7 \\
        \hline
        English & 71 & 69.8 & 71.5 & 74.0 \\
        \hline
        \hline
        Sri Lanka & 28.6 & 29 & 30.8 & 32.3 \\
        \hline
    \end{tabular}
    \caption{Computer literacy rate of Sri Lanka by Language literacy~\cite{department2019Computer,department2020Computer}}
    \label{tab:itLit}
\end{table}

\begin{table*}[!hbt]
%\begin{minipage}{\textwidth}
\centering
\begin{tabular}{lllll}
\hline
Corpus & Type & Sentence Count & Source \\
\hline
%\citet{weerasinghe-etal-2009-corpus} & Monolingual & 35.0k words & Internal Sources \\
Mozilla-I10n~\cite{tiedemann2012parallel} & Monolingual & 18.3k & Mozilla localization \\
GNOME~\cite{tiedemann2012parallel} & Parallel Multiple & 13.3k & GNOME localization \\
KDE~\cite{tiedemann2012parallel} & Parallel Multiple & 26.3k & KDE localization\\
Ubuntu~\cite{tiedemann2012parallel} & Parallel Multiple & 6.0k & Ubuntu localization \\
wikimedia~\cite{tiedemann2012parallel} & Parallel Multiple & 18.2k & Wikimedia \\
QED~\cite{abdelali2014amara} & Parallel Multiple & 4.8k & QCRI Subtitles \\ 
\citet{upeksha2015implementing,upeksha2015comparison} & Monolingual & ? & ? \\
\citet{de2015Sinhala} & Monolingual & ? & Web crawled (News)  \\
OpenSubtitles~\cite{lison2018opensubtitles2018} & Parallel Multiple & 1.0M & opensubtitles\\
\citet{guzman2019flores} & Parallel English & 8.6k & Wikipedia \\
WikiMatrix~\cite{schwenk2019wikimatrix} & Parallel Multiple & 0.3M & Wikimedia\\
JW300~\cite{agic-vulic-2019-jw300} & Parallel Multiple & 0.6M & Web crawled (jw.org) \\
\citet{wijeratne2020sinhala} & Monolingual & ? & Facebook Posts \\
ParaCrawl~\cite{banon2020paracrawl} & Parallel English & 0.2M & Web crawled (General) \\
CCAligned~\cite{el-kishky-etal-2020-ccaligned} & Parallel English & 0.6M & Web crawled (General)  \\
TED2020~\cite{reimers-gurevych-2020-making} & Parallel Multiple & 1.0k & TED \& TED-X transcripts \\
CCMatrix~\cite{fan2021beyond} & Parallel Multiple & 7.7M & Web crawled (General)    \\
XLEnt~\cite{el2021xlent} & Parallel Multiple & 0.6M & \textit{WikiMatrix}, \textit{CCMatrix}, \textit{CCAligned}
 \\
% 
\end{tabular}
\caption{Corpora}
\label{tab:corpora}
%\end{minipage}
\end{table*}

==> TikizPlot_backup.tex <==
\iffalse

\begin{figure*}[!htb]
    \centering
    \begin{tikzpicture}
    \pgfplotsset{
width=0.97\textwidth,
height=0.3\textwidth
}
\begin{axis} [ybar,
xticklabel style = {rotate=45,anchor=east},
restrict x to domain=1989:2021
]
\addplot table[ignore chars={(,)},col sep=comma]{images/paperFreq.txt};
\end{axis}
\end{tikzpicture}
    \caption{Caption}
    \label{fig:SinPapers}
\end{figure*}

\begin{figure*}[!htb]
    \centering
\begin{tikzpicture}
\pgfplotsset{
width=0.97\textwidth,
height=0.99\textwidth
}
\begin{axis}[%
scatter/classes={%
    0={fill=black!50!white,draw=black!50!black},
    1={fill=red!50!white,draw=red!50!black},
    2={fill=blue!50!white,draw=blue!50!black},
    3={fill=green!50!white,draw=green!50!black},
    4={fill=yellow!50!white,draw=yellow!50!black},
    5={fill=brown!50!white,draw=brown!50!black}
    },xlabel={CC-Count (Log)},
    ylabel={Wiki-Count (Log)}]
\addplot[scatter,only marks,mark=*,mark options={scale=2},%
    scatter src=explicit symbolic
        , nodes near coords*={\Label},
        visualization depends on={value \thisrow{label} \as \Label}
        ]%
table[x index=0,y index=1,col sep=space,meta=class] {images/CCvsWiki.csv};
%table[x index=1,y index=2,col sep=space,meta=class] {images/CCvsWikivsACL-kMeanClasses.csv};
%table[x index=0,y index=1,col sep=space,meta=class] {images/CCvsWikivsACL-zscore-kMeanClasses.csv};
%table[x index=6,y index=7, col sep=comma,meta=Joshi-Class] {images/CC_Wiki_ACL.csv};
\end{axis}
\end{tikzpicture}
    \caption{CCvsWiki}
    \label{fig:CCvsWiki}
\end{figure*}


\begin{figure*}[!htb]
    \centering
\begin{tikzpicture}
\pgfplotsset{
width=0.97\textwidth,
height=0.99\textwidth
}
\begin{axis}[%
scatter/classes={%
    0={fill=black!50!white,draw=black!50!black},
    1={fill=red!50!white,draw=red!50!black},
    2={fill=blue!50!white,draw=blue!50!black},
    3={fill=green!50!white,draw=green!50!black},
    4={fill=yellow!50!white,draw=yellow!50!black},
    5={fill=brown!50!white,draw=brown!50!black}
    },xlabel={Wiki-Count (Log)},
    ylabel={ACL-Count (Log)}]
\addplot[scatter,only marks,mark=*,mark options={scale=2},%
    scatter src=explicit symbolic
        , nodes near coords*={\WikiTag},
        visualization depends on={value \thisrow{Wiki-Tag} \as \WikiTag}
        ]%
%table[x index=5,y index=6,col sep=comma,meta=Kmean] {images/CC_Wiki_ACL.csv};
table[x index=12,y index=7, col sep=comma,meta=Kmean] {images/CC_Wiki_ACL.csv};
\end{axis}
\end{tikzpicture}
    \caption{New Graph}
    \label{fig:WikivsACL}
\end{figure*}


\begin{figure*}[!htb]
    \centering
\begin{tikzpicture}
\pgfplotsset{
width=0.97\textwidth,
height=0.99\textwidth
}
 \begin{axis}[%
scatter/classes={%
    0={fill=black!50!white,draw=black!50!black},
    1={fill=red!50!white,draw=red!50!black},
    2={fill=blue!50!white,draw=blue!50!black},
    3={fill=green!50!white,draw=green!50!black},
    4={fill=yellow!50!white,draw=yellow!50!black},
    5={fill=brown!50!white,draw=brown!50!black}
    },xlabel={CC-Count (Log)},
    ylabel={Wiki-Count (Log)},
    zlabel={ACL-Count (Log)}]
     \addplot3 [surf,only marks,mark=*,mark options={scale=1},%
    scatter src=explicit symbolic
        , nodes near coords*={\WikiTag},
        visualization depends on={value \thisrow{Wiki-Tag} \as \WikiTag}]
  table[x index=5,y index=7, y index=6, col sep=comma,meta=Kmean] {images/CC_Wiki_ACL.csv};
\end{axis}
 \end{tikzpicture}
   \caption{CCvsWikivsACL}
    \label{fig:CCvsWikivsACL}
\end{figure*}

\fi

==> headder.tex <==
\usepackage[utf8]{inputenc}
\usepackage{graphicx}

\usepackage[numbers,sort&compress]{natbib}

\usepackage{hyperref}
\hypersetup{
colorlinks   = true,
citecolor    = blue,
urlcolor    =  blue
}

%\usepackage{fontspec}
%\newfontfamily{\Japanese}{simsun.ttc}[Language=Japanese]
%\newfontfamily{\sinhala}{ISKPOTA.TTF}[Language=Sinhala]
%\usepackage{lscape}

\usepackage{url}
\usepackage{cleveref}
\crefformat{footnote}{#2\footnotemark[#1]#3}

\newcommand{\footURL}[1]{\footnote{\url{#1}}}
\newcommand{\footURLcl}[2]{\footnote{\label{#2}\url{#1}}}

\usepackage{ragged2e}

\usepackage[
singlelinecheck=false % <-- important
]{caption}
\usepackage{multirow}
\usepackage{hhline}
\usepackage{subcaption}

\usepackage{ftnxtra}
\usepackage{fnpos}




%This command block allows partial inserting of files
% Taken from https://tex.stackexchange.com/questions/4889/input-only-part-of-a-file
\makeatletter
\newread\pin@file
\newcounter{pinlineno}
\newcommand\pin@accu{}
\newcommand\pin@ext{pintmp}
% inputs #3, selecting only lines #1 to #2 (inclusive)
\newcommand*\partialinput [3] {%
  \IfFileExists{#3}{%
    \openin\pin@file #3
    % skip lines 1 to #1 (exclusive)
    \setcounter{pinlineno}{1}
    \@whilenum\value{pinlineno}<#1 \do{%
      \read\pin@file to\pin@line
      \stepcounter{pinlineno}%
    }
    % prepare reading lines #1 to #2 inclusive
    \addtocounter{pinlineno}{-1}
    \let\pin@accu\empty
    \begingroup
    \endlinechar\newlinechar
    \@whilenum\value{pinlineno}<#2 \do{%
      % use safe catcodes provided by e-TeX's \readline
      \readline\pin@file to\pin@line
      \edef\pin@accu{\pin@accu\pin@line}%
      \stepcounter{pinlineno}%
    }
    \closein\pin@file
    \expandafter\endgroup
    \scantokens\expandafter{\pin@accu}%
  }{%
    \errmessage{File `#3' doesn't exist!}%
  }%
}
\makeatother

\newcommand{\version}{\partialinput{1}{1}{ReleaseNotes.txt}}

\usepackage{pdflscape}
\usepackage{svg}


==> surveyGraphs.tex <==
\newcommand{\SurveyGraph}[3]{
\begin{figure*}[!hbt]
     \centering
     \begin{subfigure}[!hbt]{0.99\textwidth}
         \centering
         \includegraphics[height=15pt,keepaspectratio]{images/#3_#1_Axis.png}
     \end{subfigure}
     
     \begin{subfigure}[!hbt]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/#3_#1.png}
         \caption{#2 Count}
         \label{fig:#1_count}
     \end{subfigure}
     \hfill
     \begin{subfigure}[!hbt]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/#3_#1_Cumulative_Percentage.png}
         \caption{#2 Percentage Cumulative}
         \label{fig:#1_cumulative}
     \end{subfigure}
        \caption{#2 analysis from the papers listed in~\cite{de2019survey}}
        \label{fig:#1}
\end{figure*}
}
